Let's Go Real Talk: Spoken Dialogue Model for Face-to-Face Conversation

In this paper, we introduce a novel Face-to-Face spoken dialogue model. It processes audio-visual speech from user input and generates audio-visual speech as the response, marking the initial step towards creating an avatar chatbot system without relying on intermediate text. To this end, we newly introduce MultiDialog, the first large-scale multimodal (i.e., audio and visual) spoken dialogue corpus containing 340 hours of approximately 9,000 dialogues, recorded based on the open domain dialogue dataset, TopicalChat. The MultiDialog contains parallel audio-visual recordings of conversation partners acting according to the given script with emotion annotations, which we expect to open up research opportunities in multimodal synthesis. Our Face-to-Face spoken dialogue model incorporates a textually pretrained large language model and adapts it into the audio-visual spoken dialogue domain by incorporating speech-text joint pretraining. Through extensive experiments, we validate the effectiveness of our model in facilitating a face-to-face conversation. Demo and data are available at https://multidialog.github.io and https://huggingface.co/datasets/IVLLab/MultiDialog, respectively.

==> tables/table3.tex <==
\begin{table}
	\renewcommand{\arraystretch}{1.2}
	\renewcommand{\tabcolsep}{2mm}
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{lcc}
\Xhline{3\arrayrulewidth}
\multicolumn{1}{p{5cm}}{\textbf{Method}} & 
\multicolumn{1}{p{1.8cm}}{\centering \textbf{N-MOS} \uparrow} & 
\multicolumn{1}{p{1.8cm}}{\centering \textbf{M-MOS} \downarrow} \\
\hline
\multicolumn{3}{l}{\quad $\bullet$ \textbf{\textit{Ground Truth}}} \\ 
GT Video &   \\
GT Audio-Visual Unit &  \\
\hdashline

\multicolumn{3}{l}{\quad $\bullet$ \textbf{\textit{Speech Dialogue System}}} \\ 
SpeechGPT \cite{zhang2023speechgpt} & \\
d-GSLM \cite{nguyen2023generative} & \\
\hdashline

\multicolumn{3}{l}{\quad $\bullet$ \textbf{\textit{Cascade System}}} \\ 
AVSR + LM + TTS + TFG &\\
\hdashline

\multicolumn{3}{l}{\quad $\bullet$ \textbf{\textit{Multimodal Speech Dialogue System}}} \\ 
% {C4} & GT AV Unit (GT duration) & 8.76  & 6.14 & 3.13 \\
Proposed &  \\
% {C5} & Translated AV Speech Unit$^\dagger$ & 6.48 & 7.92  &  1.76  \\

\Xhline{3\arrayrulewidth}
\end{tabular}}
\vspace{-0.3cm}
\caption{}
\label{table:3}
\vspace{-0.5cm}
\end{table} 
